Hexahedral mesh of anatomical atlas for construction of computational human brain models: Applications to modeling biomechanics and bioelectric field propagation

Numerical simulations rely on constructing accurate and detailed models to produce reliable results - a task that is often challenging. This task becomes notably more difficult when the model is of the human brain. We create an anatomically comprehensive hexahedral mesh of the human brain using an open-source digital brain atlas. Digital atlases are valuable tools currently used by medical professionals, medical students, and researchers for gathering, presenting, and discovering knowledge about the human brain. We demonstrate that the atlas can be used to efficiently create an accurate and detailed hexahedral finite element mesh of the brain for scientific computing. We present two case studies. The first case study constructs a biomechanical model of the brain to compute brain deformations and predict traumatic brain injury risk due to violent impact. In the second case study, we construct a bioelectrical model of the brain to solve the electroencephalography (EEG) forward problem, a frequent simulation process used in electrophysiology to study electromagnetic fields generated by the nervous system. We demonstrate efficient and accurate model construction using the meshed anatomical brain atlas, as well as emphasize the importance of effective communication and contextual analysis of results for enabling multi-disciplinary scientific computing research.

==> results.tex <==
\subsection{Visualisation of Simulation Results}

To display the simulation results with reference to the anatomical structures, we used ParaView, an open-source software for volume rendering and scientific visualization. Figure 4 show the electric potential field obtained from the dipole source with reference to the anatomical labels of the atlas. Our method offers users the ability to query results and their statistics by anatomical labels compared to previous methods that only used spatial coordinates, element number or node number. This provides additional information about the affected brain area, aiding researchers and medical professionals. We demonstrate this in Figure 5 by visualising the electric potential on the left middle temporal gyrus and its substructures.

%FIG4

%FIG5

\subsection{Simulation results}
We demonstrate the benefits of using an atlas-based mesh by querying simulation results from specific regions of the brain, specifically the left middle temporal gyrus, where the dipole is located. We also query anatomical substructures, including the amygdala, parahippocampal gyrus, and fusiform gyrus, as these regions are typically implicated in the temporal lobe epilepsy seizure activity [17]. This approach holds significance since electro-physiological assessments primarily guide the decision-making process for surgical intervention in TLE patients [18]. 

We examine the maximum, minimum and mean potentials at the locations detailed in Table 2 below.

%TABLE2


